A Partial Decode-Forward Scheme For A Network with N relays

We study a discrete-memoryless relay network consisting of one source, one destination and N relays, and design a scheme based on partial decode-forward relaying. The source splits its message into one common and N+1 private parts, one intended for each relay. It encodes these message parts using Nth-order block Markov coding, in which each private message part is independently superimposed on the common parts of the current and N previous blocks. Using simultaneous sliding window decoding, each relay fully recovers the common message and its intended private message with the same block index, then forwards them to the following nodes in the next block. This scheme can be applied to any network topology. We derive its achievable rate in a compact form. The result reduces to a known decode-forward lower bound for an N-relay network and partial decode-forward lower bound for a two-level relay network. We then apply the scheme to a Gaussian two-level relay network and obtain its capacity lower bound considering power constraints at the transmitting nodes.

==> reflist.tex <==
@ARTICLE{aref2011SSRN,
author={L. Ghabeli and M. R. Aref},
journal={IEEE Trans. on Info. Theory},
title={Symmertric semideterministic relay networks with no interference at the relays},
year={2011},
month={September},
volume={57},
number={9},
pages={5673-5681},
}

@ARTICLE{ahlswede2000networkInfoFlow,
author={R. Ahlswede, N. Cai, S.-Y. R. Li and R. W. Yeung},
journal={IEEE Trans. on Info. Theory},
title={Network information flow},
year={2000},
month={July},
volume={46},
number={4},
pages={1204-1216},
}

@ARTICLE{gastpar2005large_gaussian_RN,
author={M. Gastpar and M. Vetterli},
journal={IEEE Trans. on Info. Theory},
title={On the capacity of large \uppercase{G}aussian relay networks},
year={2005},
month={March},
volume={51},
number={3},
pages={765-779},
}

@ARTICLE{arefPDF,
author={A. El Gamal and M. R. Aref},
journal={IEEE Trans. on Info. Theory},
title={The capacity of the semideterministic relay channel},
year={1982},
volume={28},
number={3},
pages={536},
}

@INPROCEEDINGS{aref2009pdftwolevel,
author={L. Ghabeli and M. R. Aref},
booktitle={IEEE Int'l Symp. on Info. Theory (ISIT)},
title={Simultaneous partial and backward decoding approach for two-level relay networks},
year={2009},
month={June},
volume={},
number={},
}

@INPROCEEDINGS{aref2010pdftwolevel,
author={L. Ghabeli and M. R. Aref},
booktitle={IEEE Int'l Symp. on Info. Theory (ISIT)},
title={On achievable rate for relay networks based on partial decode-and-forward},
year={2010},
month={June},
volume={},
number={},
}

@INPROCEEDINGS{aref2007pdfnetwork,
author={L. Ghabeli and M. R. Aref},
booktitle={IEEE Int'l Symp. on Info. Theory (ISIT)},
title={A new achievable rate and the capacity of a class of semideterministic relay networks},
year={2007},
month={June},
volume={},
number={},
}

@ARTICLE{Xie2005multilevelrelay,
author={Xie, L.-L. and P. R. Kumar},
journal={IEEE Trans. on Info. Theory},
title={An achievable rate for the multiple level relay channel},
year={2005},
month={April},
volume={51},
number={4},
pages={1348-1358},
}

@book{gamal2010lecture,
  title={Network information theory},
  author={Abbas El Gamal and Young-Han Kim},
  year={2011},
  publisher={Cambridge University Press}
}

@INPROCEEDINGS{Ramalingam2011superposition,
author={Ramalingam, N. and Zhengdao Wang},
booktitle={IEEE Int'l Symp. on Info. Theory (ISIT)},
title={Superposition Noisy Network Coding},
year={2011},
month={Aug.},
volume={},
number={},
}

@INPROCEEDINGS{Luo2011on,
author={Luo, Kevin and Gohary, Ramy H. and Yanikomeroglu, Halim},
booktitle={IEEE Info. Theory Workshop (ITW)},
title={On the generalization of decode-and-forward and compress-and-forward for  \uppercase{G}aussian relay channels},
year={2011},
month={Oct.},
volume={},
number={},
keywords={},
doi={10.1109/ITW.2011.6089572},
ISSN={},}

@INPROCEEDINGS{Lim2010layered,
author={Lim, Sung Hoon and Kim, Young-Han and El Gamal, Abbas and Chung, Sae-Young},
booktitle={IEEE Wireless Net. Coding Conf. (WiNC)},
title={Layered Noisy Network Coding},
year={2010},
month={June},
volume={},
number={},
keywords={},
doi={10.1109/WINC.2010.5507935},
ISSN={},}

@book{cover2006elements,
  title={Elements of Information Theory},
  author={Thomas M. Cover and Joy A. Thomas},
  year={2006},
  publisher={John Wiley}
}

@INPROCEEDINGS{Wuonallerton2010,
author={Xiugang Wu and Liang-Liang Xie},
booktitle={48th Annual Allerton Conf. on Comm., Control, and Computing},
title={On the optimality of successive decoding in compress-and-forward relay schemes},
year={2010},
month={Oct.},
volume={},
number={},
}


@ARTICLE{Kim2009quantifying,
author={Kim, T.T. and Skoglund, M. and Caire, G.},
journal={IEEE Trans. on Info. Theory},
title={Quantifying the loss of compress-forward relaying without \uppercase{W}yner-\uppercase{Z}iv coding},
year={2009},
month={April},
volume={55},
number={4},
pages={1529-1533},
}



@INPROCEEDINGS{Zhou2011incremental,
author={Lei Zhou and Wei Yu},
booktitle={49th Annual Allerton Conf. on Comm., Control, and Computing},
title={Incremental Relaying for the \uppercase{G}aussian Interference Channel with a Degraded Broadcasting Relay},
month={Sept.},
year={2011},
volume={},
number={},
}


@ARTICLE{Chong2007generalized,
author={Chong, H.-F. and Motani, M. and Garg, H. K.},
journal={IEEE Trans. on Info. Theory},
title={Generalized Backward Decoding Strategies for the Relay Channel},
year={2007},
month={Jan.},
volume={53},
number={1},
pages={394-401},
}

@article{Wu2010on,
  author    = {Xiugang Wu and
               Liang-Liang Xie},
  title     = {On the optimal compressions in the compress-and-forward relay schemes},
  journal   = {Arxiv preprint arXiv: 1009.5959v3},
  year      = {2011},

}




@ARTICLE{Kramer2005cooperative,
author={ Kramer, G. and Gastpar, M. and Gupta, P.},
journal={IEEE Trans. on Info. Theory},
title={Cooperative Strategies and Capacity Theorems for Relay Networks},
year={2005},
month={Sept.},
volume={51},
number={9},
pages={3037-3063},
}


@INPROCEEDINGS{zhong2011compress,
title={Compress-Forward without \uppercase{W}yner-\uppercase{Z}iv Binning for the One-Way and Two-Way Relay Channels
},
  author={Peng Zhong and Mai Vu},
booktitle={49th Annual Allerton Conf. on Comm., Control, and Computing},
month={Sept.},
year={2011}
}



@INPROCEEDINGS{Kramer2011short,
author={Kramer, G. and Hou, J.},
booktitle={8th Int'l Workshop on Multi-Carrier Systems Solutions (MC-SS)},
title={Short-message quantize-forward network coding},
year={2011},
month={May},
volume={},
number={},
pages={1-3},
}


@INPROCEEDINGS{Razaghi2010universal,
author={Razaghi, P. and Wei Yu},
booktitle={Info. Theory and Applications Workshop (ITA)},
title={Universal relaying for the interference channel},
year={2010},
month={Feb.},
volume={},
number={},
%pages={1-6},
}


@INPROCEEDINGS{Cover2007capacity,
author={Cover, Thomas M. and Kim, Young-Han},
booktitle={IEEE Int'l Symp. on Info. Theory (ISIT)},
title={Capacity of a Class of Deterministic Relay Channels},
year={2007},
month={June},
volume={},
number={},
pages={591-595},
keywords={},
doi={10.1109/ISIT.2007.4557289},
ISSN={},}


@INPROCEEDINGS{Kim2007coding,
author={Kim, Young-Han},
booktitle={45th Annual Allerton Conf. on Comm., Control, and Computing},
title={Coding Techniques for Primitive Relay Channels},
year={2007},
month={Sept.},
volume={},
number={},
}

@ARTICLE{Lantse,
author={Laneman, J.N. and Tse, D.N.C. and Wornell, G.W.},
journal={IEEE Trans. on Info. Theory},
title={Cooperative diversity in wireless networks: Efficient protocols and outage behavior},
year={2004},
month={Dec.},
volume={50},
number={12},
pages={3062-3080},
}


%\noindent [\label{ZEqnNum280982}] Cognitive Radio Technology - A Study for Ofcom, [online] Available: http://www.ofcom.org.uk/research

@ARTICLE{sagwei,
author={Sagias, N.C. and Zogas, D.A. and Karagiannidis, G.K. and Tombras, G.S.},
journal={IEEE Communications Letters},
title={Channel capacity and second-order statistics in \uppercase{W}eibull fading},
year={2004},
month={June},
volume={8},
number={6},
pages={377-379},
}

@book{tabofint,
  title={{Table of integrals, series, and products}},
  author={Gradshteyn, I. S. and Ryzhik, I. M.},
  year={2004},
  publisher={New York: Wiley},
}

%@book{hsce612,
%  title={{Lecture Notes on Network Information Theory}},
%  author={El Gamal, R. and  Kim, Y.-H.},
%  year={2010},
%  publisher={Available: http://arxiv.org/abs/1001.3404/},
%}


@inproceedings{gradshteyn2004table,
title={Table of integrals, series, and prducts},
author={I.S.Gradshteyn and I.M.Ryzhik},
year={2004},
organization={New York: Wiley},
}



@article{meulen1971three,
     title = {Three-Terminal Communication Channels},
     author = {van der Meulen, E.},
     journal = {Advances in Applied Probability},
     volume = {3},
     number = {1},
     year = {1971},
     pages = {120-154},
     }

@article{willems1985the,
author={Willems, F. and van der Meulen, E.},
journal={IEEE Trans. on Info. Theory},
title={The discrete memoryless multiple-access channel with cribbing encoders},
year={1985},
month={May},
volume={31},
number={3},
pages={313-327},
}

@article{Wyner1976the,
author={ Wyner, A. and Ziv, J.},
journal={IEEE Trans. on Info. Theory},
title={The rate-distortion function for source coding with side information at the decoder},
year={1976},
month={Jan.},
volume={22},
number={1},
pages={1-10},
}

@article{gamal2006bounds,
author={El Gamal, A. and Mohseni, M. and Zahedi, S.},
journal={IEEE Trans. on Info. Theory},
title={Bounds on capacity and minimum energy-per-bit for \uppercase{AWGN} relay channels},
year={2006},
month={April},
volume={52},
number={4},
pages={1545-1561},
}

%
%@article{gamal2010lecture,
%  title={Lecture Notes on Network Information Theory},
%  author={El Gamal, A. and Kim, Y.-H.},
%  journal={Arxiv preprint arXiv:1001.3404},
%  year={2010}
%}

@ARTICLE{sung2011noisy,
author={Sung Hoon Lim and Young-Han Kim and El Gamal, A. and Sae-Young Chung},
journal={IEEE Trans. on Info. Theory},
title={Noisy Network Coding},
year={2011},
month={May},
volume={57},
number={5},
pages={3132-3152},
}

@inproceedings{shannon1961two,
  title={Two-way communication channels},
  author={Shannon, C.E.},
  booktitle={Proc. 4th Berkeley Symp. Math. Stat. Prob},
  volume={1},
  pages={351-384},
  year={1961},
  organization={IEEE Press}
}

@article{cover1979capacity,
  title={Capacity theorems for the relay channel},
  author={Cover, T. and El Gamal, A.},
  journal={IEEE Trans. on Info. Theory},
  volume={25},
  number={5},
  pages={572-584},
  year={1979},
  publisher={IEEE}
}

@inproceedings{rankov2006achievable,
  title={Achievable rate regions for the two-way relay channel},
  author={Rankov, B. and Wittneben, A.},
  booktitle={IEEE Int'l Symp. on Info. Theory (ISIT)},
  year={2006},

}

@inproceedings{xie2007network,
  title={Network coding and random binning for multi-user channels},
  author={Xie, L.L.},
  booktitle={10th Canadian Workshop on Info. Theory (CWIT)},
  pages={85-88},

  year={2007}
}

@inproceedings{narayanan2007joint,
  title={Joint physical layer coding and network coding for bi-directional relaying},
  author={Narayanan, K. and Wilson, M.P. and Sprintson, A.},
  booktitle={45th Annual Allerton Conf. on Comm., Control, and Computing},
  year={2007}
}

@inproceedings{nam2008capacity,
  title={Capacity bounds for two-way relay channels},
  author={Nam, W. and Chung, S.Y. and Lee, Y.H.},
  booktitle={IEEE Int'l Zurich Seminar on Communications},
  pages={144-147},
  year={2008},
  organization={IEEE}
}

@article{erez2004achieving,
  title={Achieving 1/2 log (1+ SNR) on the \uppercase{AWGN} channel with lattice encoding and decoding},
  author={Erez, U. and Zamir, R.},
  journal={IEEE Trans. on Info. Theory},
  volume={50},
  number={10},
  pages={2293-2314},
  year={2004},
  publisher={IEEE}
}

@article{erez2005lattices,
  title={Lattices which are good for (almost) everything},
  author={Erez, U. and Litsyn, S. and Zamir, R.},
  journal={IEEE Trans. on Info. Theory},
  volume={51},
  number={10},
  pages={3401-3416},
  year={2005},
  publisher={IEEE}
}

@article{nam2009capacity,
  title={Capacity of the \uppercase{g}aussian two-way relay channel to within 1/2 bit},
  author={Nam, W. and Chung, S.Y. and Lee, Y.H.},
  journal={IEEE Trans. on Info. Theory},
  volume={56},
  number={11},
  pages={5488-5494},
  year={2010},
  publisher={IEEE}
}

@article{nazer2009compute,
  title={Compute-and-forward: Harnessing interference through structured codes},
  author={Nazer, B. and Gastpar, M.},
  journal={Arxiv preprint arXiv:0908.2119},
  year={2009}
}

@inproceedings{song2010list,
  title={List decoding for nested lattices and applications to relay channels},
  author={Song, Y. and Devroye, N.},
  booktitle={48th Annual Allerton Conf. on Comm., Control, and Computing},
  pages={1038-1045},
  year={2010},
  organization={IEEE}
}

